Odyssey: An Interactive Workbench for Expert-Driven Floating-Point Expression Rewriting

In recent years, researchers have proposed a number of automated tools to identify and improve floating-point rounding error in mathematical expressions. However, users struggle to effectively apply these tools. In this paper, we work with novices, experts, and tool developers to investigate user needs during the expression rewriting process. We find that users follow an iterative design process. They want to compare expressions on multiple input ranges, integrate and guide various rewriting tools and understand where errors come from. We organize this investigation's results into a three-stage workflow and implement that workflow in a new, extensible workbench dubbed Odyssey. Odyssey enables users to: (1) diagnose problems in an expression, (2) generate solutions automatically or by hand, and (3) tune their results. Odyssey tracks a working set of expressions and turns a state-of-the-art automated tool "inside out," giving the user access to internal heuristics, algorithms, and functionality. In a user study, Odyssey enabled five expert numerical analysts to solve challenging rewriting problems where state-of-the-art automated tools fail. In particular, the experts unanimously praised Odyssey's novel support for interactive range modification and local error visualization.

==> conclusion.tex <==
\section{Conclusion}

Odyssey's design,
  grounded in an explicit workflow model
  and validated on real-world tasks,
  allows users to take advantage of automated tools
  without feeling constrained by them.
Its extensible architecture will allow it to grow
  to address
  a variety of floating-point expression rewriting problems,
  ultimately improving the quality of results across various fields. 
